SCMO: Stochastic Control for Optimization over Probability Measures on Infinite-Dimensional Spaces

We study objective-only optimization of possibly nonconvex and nonsmooth functionals over probability measures on a separable Hilbert space, allowing the optimizer to be intrinsically non-Dirac. We introduce SCMO (Stochastic Control Measure Optimizer), a gradient-free particle method derived from entropy regularized stochastic control. After finite-particle and Galerkin approximations, a Cole--Hopf transform represents the optimal feedback as a Gibbs-weighted terminal displacement. SCMO approximates this feedback by sampling context clouds, replacing one particle at a time with candidate draws, scoring the resulting empirical measures, and applying exponential reweighting. SCMO uses separate covariances for candidate proposals and particle updates, termed matched when equal and nonmatched otherwise; our analysis covers both settings. In the matched case, we establish PDE-free qualitative convergence and a projection-first quantitative bound separating particle, Galerkin-projection, and entropy-regularization errors. For the practical multi-context implementation with nonmatched covariance, we prove finite-candidate consistency and show that the signed, curvature-dependent effect of nonmatched covariance can reduce the resulting upper bound on the approximation error. Finally, experiments on function-space, trajectory-law, and contact-rich manipulation problems show that SCMO handles nonsmooth and nonconvex objectives, escapes suboptimal local basins, and recovers prescribed multimodal, non-Dirac law structure. Code for reproducing our experimental results is available at https://github.com/HenryCHEUNG7373/SCMO.

==> graphs/unmatched_covariance/summary_table.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\caption{Curvature diagnostic for fixed nonmatched execution covariance over 50 independent runs. Negative $\mathcal C=-\mathcal G+\mathcal P$ is favorable; negative $\mathcal E+\mathcal C$ means that the gain also dominates the Euler residual.}
\label{tab:unmatched-curvature-diagnostic}
\begin{tabular}{lrrrrrrr}
\toprule
Initialization & $\alpha_0$ & Final $G$ & $\mathcal G$ & $\mathcal{P}$ & $\mathcal C$ & $\mathcal E+\mathcal C$ & Sign agr. \\
\midrule
barrier & 0.25 & 0.1896 $\pm$ 0.003749 & 0.001428 & 0.05052 & 0.04909 & 0.04967 & 0.999 \\
 & 0.50 & 0.1619 $\pm$ 0.004897 & 0.00355 & 0.02788 & 0.02433 & 0.02485 & 0.999 \\
 & 1.00 & 0.1359 $\pm$ 0.005757 & 0 & 0 & 0 & 0.0005928 & -- \\
 & 1.50 & 0.1269 $\pm$ 0.006398 & 0.0192 & 0.01319 & -0.006011 & -0.005289 & 0.997 \\
 & 2.00 & 0.1267 $\pm$ 0.007468 & 0.03442 & 0.03374 & -0.00068 & 0.0001851 & 0.996 \\
\addlinespace
well & 0.25 & 0.02055 $\pm$ 0.001712 & 0.08137 & 3.023e-05 & -0.08134 & -0.07982 & 1.000 \\
 & 0.50 & 0.03843 $\pm$ 0.003048 & 0.05316 & 0.0002451 & -0.05291 & -0.05134 & 1.000 \\
 & 1.00 & 0.0705 $\pm$ 0.005405 & 0 & 0 & 0 & 0.001691 & -- \\
 & 1.50 & 0.09788 $\pm$ 0.008226 & 0.002241 & 0.05093 & 0.04869 & 0.0505 & 0.999 \\
 & 2.00 & 0.1221 $\pm$ 0.01152 & 0.006136 & 0.1011 & 0.09495 & 0.09687 & 0.999 \\
\addlinespace
\bottomrule
\end{tabular}
\end{table}

